How Well Do Sparse Imagenet Models Transfer?

Transfer learning is a classic paradigm by which models pretrained on large "upstream" datasets are adapted to yield good results on "downstream" specialized datasets. Generally, more accurate models on the "upstream" dataset tend to provide better transfer accuracy "downstream". In this work, we perform an in-depth investigation of this phenomenon in the context of convolutional neural networks (CNNs) trained on the ImageNet dataset, which have been pruned - that is, compressed by sparsifying their connections. We consider transfer using unstructured pruned models obtained by applying several state-of-the-art pruning methods, including magnitude-based, second-order, re-growth, lottery-ticket, and regularization approaches, in the context of twelve standard transfer tasks. In a nutshell, our study shows that sparse models can match or even outperform the transfer performance of dense models, even at high sparsities, and, while doing so, can lead to significant inference and even training speedups. At the same time, we observe and analyze significant differences in the behaviour of different pruning methods.

==> tables/rn50_full_all.tex <==
\begin{table}[htb!]
\centering
\scalebox{0.9}{%\
\begin{tabular}{ccccccccc}
\toprule
{Pruning Strategy} & {Dense} & {AC/DC} & {GMP} & {LTH-T} & {RigL ERK 1x} & {RigL ERK 5x} & {STR} & {WoodFisher} \\
\midrule
{80\% Sparsity} & {} & {} & {} & {} & {} & {} & {} & {}\\
\midrule

Aircraft & 83.6 $ \pm $ 0.4 & 83.3 $ \pm $ 0.1 & \textbf{84.4 $ \pm $ 0.2} & \textbf{84.7 $ \pm $ 0.5} & 82.6 $ \pm $ 0.3 & 82.4 $ \pm $ 0.2 & 79.8 $ \pm $ 0.3 & \textbf{84.8 $ \pm $ 0.2} \\

Birds & 72.4 $ \pm $ 0.3 & 69.9 $ \pm $ 0.2 & 72.5 $ \pm $ 0.2 & 71.4 $ \pm $ 0.1 & 72.3 $ \pm $ 0.3 & \textbf{73.4 $ \pm $ 0.1} & 68.1 $ \pm $ 0.1 & 72.4 $ \pm $ 0.4 \\

CIFAR-10 & \textbf{97.4 $ \pm $ 0.0} & 96.9 $ \pm $ 0.1 & 97.2 $ \pm $ 0.0 & 97.0 $ \pm $ 0.0 & 96.9 $ \pm $ 0.0 & 97.1 $ \pm $ 0.0 & 96.5 $ \pm $ 0.1 & 97.2 $ \pm $ 0.1 \\

CIFAR-100 & \textbf{85.6 $ \pm $ 0.2} & 84.9 $ \pm $ 0.2 & 85.1 $ \pm $ 0.0 & 84.4 $ \pm $ 0.2 & 83.6 $ \pm $ 0.2 & 84.1 $ \pm $ 0.4 & 83.6 $ \pm $ 0.2 & 85.1 $ \pm $ 0.1 \\
Caltech-101 & \textbf{93.5 $ \pm $ 0.1} & 92.5 $ \pm $ 0.2 & \textbf{93.7 $ \pm $ 0.5} & 92.1 $ \pm $ 0.5 & 92.5 $ \pm $ 0.1 & 92.0 $ \pm $ 0.3 & 90.7 $ \pm $ 0.6 & \textbf{93.7 $ \pm $ 0.1} \\

Caltech-256 & \textbf{86.1 $ \pm $ 0.1} & 85.4 $ \pm $ 0.2 & 85.1 $ \pm $ 0.2 & 83.1 $ \pm $ 0.1 & 83.8 $ \pm $ 0.1 & 84.2 $ \pm $ 0.2 & 84.0 $ \pm $ 0.1 & 85.1 $ \pm $ 0.1 \\

Cars & \textbf{90.3 $ \pm $ 0.2} & 89.2 $ \pm $ 0.1 & \textbf{90.3 $ \pm $ 0.1} & 89.9 $ \pm $ 0.0 & 89.4 $ \pm $ 0.1 & 89.6 $ \pm $ 0.1 & 87.8 $ \pm $ 0.1 & \textbf{90.5 $ \pm $ 0.2} \\

DTD & \textbf{76.2 $ \pm $ 0.3} & 75.7 $ \pm $ 0.5 & 75.4 $ \pm $ 0.1 & 75.2 $ \pm $ 0.4 & 74.5 $ \pm $ 0.2 & 74.2 $ \pm $ 0.2 & 73.7 $ \pm $ 0.6 & 75.4 $ \pm $ 0.3 \\

Flowers & 95.0 $ \pm $ 0.1 & 94.7 $ \pm $ 0.2 & 95.9 $ \pm $ 0.2 & 93.9 $ \pm $ 0.2 & 95.7 $ \pm $ 0.2 & \textbf{96.1 $ \pm $ 0.1} & 93.7 $ \pm $ 0.2 & 95.5 $ \pm $ 0.2 \\

Food-101 & \textbf{87.3 $ \pm $ 0.1} & 86.9 $ \pm $ 0.1 & \textbf{87.4 $ \pm $ 0.1} & 86.9 $ \pm $ 0.1 & 86.9 $ \pm $ 0.1 & \textbf{87.2 $ \pm $ 0.1} & 85.9 $ \pm $ 0.1 & \textbf{87.4 $ \pm $ 0.1} \\

Pets & \textbf{93.4 $ \pm $ 0.1} & 92.5 $ \pm $ 0.0 & \textbf{93.4 $ \pm $ 0.1} & 92.9 $ \pm $ 0.1 & 92.2 $ \pm $ 0.1 & 92.4 $ \pm $ 0.1 & 92.1 $ \pm $ 0.1 & \textbf{93.3 $ \pm $ 0.3} \\

SUN397 & \textbf{64.8 $ \pm $ 0.0} & 64.0 $ \pm $ 0.0 & 63.1 $ \pm $ 0.1 & 61.7 $ \pm $ 0.2 & 62.2 $ \pm $ 0.2 & 62.0 $ \pm $ 0.3 & 62.6 $ \pm $ 0.1 & 62.8 $ \pm $ 0.1 \\

\midrule
{90\% Sparsity} & {} & {} & {} & {} & {} & {} & {} & {} \\
\midrule

Aircraft & 83.6 $ \pm $ 0.4 & 82.8 $ \pm $ 1.0 & \textbf{83.9 $ \pm $ 0.7} & \textbf{84.9 $ \pm $ 0.3} & 81.6 $ \pm $ 0.5 & 83.0 $ \pm $ 0.4 & 78.7 $ \pm $ 0.4 & \textbf{84.5 $ \pm $ 0.4} \\
Birds & \textbf{72.4 $ \pm $ 0.3} & 68.5 $ \pm $ 0.1 & 70.5 $ \pm $ 0.1 & 67.8 $ \pm $ 0.2 & 70.3 $ \pm $ 0.0 & \textbf{72.9 $ \pm $ 0.2} & 66.0 $ \pm $ 0.2 & 71.6 $ \pm $ 0.2 \\
CIFAR-10 & \textbf{97.4 $ \pm $ 0.0} & 96.6 $ \pm $ 0.1 & 97.1 $ \pm $ 0.0 & 96.6 $ \pm $ 0.2 & 96.4 $ \pm $ 0.1 & 97.0 $ \pm $ 0.1 & 96.1 $ \pm $ 0.1 & 97.0 $ \pm $ 0.1 \\
CIFAR-100 & \textbf{85.6 $ \pm $ 0.2} & 83.9 $ \pm $ 0.1 & 84.4 $ \pm $ 0.0 & 83.0 $ \pm $ 0.1 & 83.0 $ \pm $ 0.2 & 83.7 $ \pm $ 0.3 & 82.9 $ \pm $ 0.2 & 84.4 $ \pm $ 0.2 \\
Caltech-101 & \textbf{93.5 $ \pm $ 0.1} & 92.6 $ \pm $ 0.2 & 92.9 $ \pm $ 0.2 & 84.5 $ \pm $ 0.3 & 91.7 $ \pm $ 0.3 & 92.3 $ \pm $ 0.4 & 90.9 $ \pm $ 0.3 & \textbf{93.9 $ \pm $ 0.3} \\
Caltech-256 & \textbf{86.1 $ \pm $ 0.1} & 84.8 $ \pm $ 0.1 & 83.7 $ \pm $ 0.3 & 78.6 $ \pm $ 0.1 & 82.7 $ \pm $ 0.2 & 84.0 $ \pm $ 0.1 & 83.1 $ \pm $ 0.2 & 84.0 $ \pm $ 0.1 \\
Cars & \textbf{90.3 $ \pm $ 0.2} & 88.5 $ \pm $ 0.2 & 89.5 $ \pm $ 0.0 & 89.5 $ \pm $ 0.1 & 88.4 $ \pm $ 0.1 & 89.2 $ \pm $ 0.1 & 86.7 $ \pm $ 0.2 & \textbf{90.0 $ \pm $ 0.2} \\
DTD & \textbf{76.2 $ \pm $ 0.3} & 75.2 $ \pm $ 0.1 & 74.2 $ \pm $ 0.1 & 71.9 $ \pm $ 0.1 & 73.4 $ \pm $ 0.4 & 75.2 $ \pm $ 0.8 & 73.2 $ \pm $ 0.4 & 75.5 $ \pm $ 0.4 \\
Flowers & 95.0 $ \pm $ 0.1 & 94.6 $ \pm $ 0.1 & 95.3 $ \pm $ 0.1 & 89.8 $ \pm $ 0.2 & 95.5 $ \pm $ 0.1 & \textbf{96.1 $ \pm $ 0.1} & 93.4 $ \pm $ 0.4 & 95.5 $ \pm $ 0.3 \\
Food-101 & \textbf{87.3 $ \pm $ 0.1} & 86.6 $ \pm $ 0.1 & 86.8 $ \pm $ 0.1 & 86.4 $ \pm $ 0.1 & 85.9 $ \pm $ 0.1 & \textbf{87.3 $ \pm $ 0.2} & 84.8 $ \pm $ 0.0 & \textbf{87.0 $ \pm $ 0.1} \\
Pets & \textbf{93.4 $ \pm $ 0.1} & 92.1 $ \pm $ 0.1 & 92.2 $ \pm $ 0.1 & 91.1 $ \pm $ 0.2 & 91.4 $ \pm $ 0.2 & 92.3 $ \pm $ 0.1 & 91.7 $ \pm $ 0.2 & 92.7 $ \pm $ 0.3 \\
SUN397 & \textbf{64.8 $ \pm $ 0.0} & 63.0 $ \pm $ 0.0 & 62.5 $ \pm $ 0.2 & 58.3 $ \pm $ 0.2 & 61.3 $ \pm $ 0.1 & 62.0 $ \pm $ 0.2 & 61.2 $ \pm $ 0.0 & 62.3 $ \pm $ 0.1 \\

\midrule
{95\% Sparsity} & {} & {} & {} & {} & {} & {} & {} \\
\midrule
Aircraft & \textbf{83.6 $ \pm $ 0.4} & 81.2 $ \pm $ 0.4 & {N \slash A} & 82.6 $ \pm $ 0.8 & 80.7 $ \pm $ 0.1 & 82.5 $ \pm $ 0.4 & 76.7 $ \pm $ 0.8 & \textbf{83.6 $ \pm $ 0.6} \\
Birds & \textbf{72.4 $ \pm $ 0.3} & 66.9 $ \pm $ 0.1 & {N \slash A} & 62.2 $ \pm $ 0.1 & 68.3 $ \pm $ 0.2 & 71.6 $ \pm $ 0.1 & 62.3 $ \pm $ 0.1 & 69.9 $ \pm $ 0.1 \\
CIFAR-10 & \textbf{97.4 $ \pm $ 0.0} & 96.2 $ \pm $ 0.1 & {N \slash A} & 95.5 $ \pm $ 0.1 & 96.0 $ \pm $ 0.1 & 96.6 $ \pm $ 0.1 & 95.4 $ \pm $ 0.1 & 96.7 $ \pm $ 0.1 \\
CIFAR-100 & \textbf{85.6 $ \pm $ 0.2} & 82.9 $ \pm $ 0.1 & {N \slash A} & 80.0 $ \pm $ 0.1 & 82.0 $ \pm $ 0.2 & 82.8 $ \pm $ 0.0 & 80.9 $ \pm $ 0.3 & 83.1 $ \pm $ 0.1 \\
Caltech-101 & \textbf{93.5 $ \pm $ 0.1} & 91.9 $ \pm $ 0.2 & {N \slash A} & 65.3 $ \pm $ 0.8 & 90.7 $ \pm $ 0.4 & 92.2 $ \pm $ 0.3 & 89.8 $ \pm $ 0.1 & 92.0 $ \pm $ 0.3 \\
Caltech-256 & \textbf{86.1 $ \pm $ 0.1} & 83.1 $ \pm $ 0.0 & {N \slash A} & 71.8 $ \pm $ 0.3 & 81.1 $ \pm $ 0.2 & 83.1 $ \pm $ 0.2 & 80.3 $ \pm $ 0.0 & 82.4 $ \pm $ 0.1 \\
Cars & \textbf{90.3 $ \pm $ 0.2} & 87.6 $ \pm $ 0.1 & {N \slash A} & 87.5 $ \pm $ 0.4 & 87.9 $ \pm $ 0.3 & 88.9 $ \pm $ 0.2 & 84.9 $ \pm $ 0.2 & 88.9 $ \pm $ 0.2 \\
DTD & \textbf{76.2 $ \pm $ 0.3} & 74.1 $ \pm $ 0.4 & {N \slash A} & 67.1 $ \pm $ 0.8 & 73.3 $ \pm $ 0.2 & 73.5 $ \pm $ 0.2 & 72.6 $ \pm $ 0.4 & 73.7 $ \pm $ 0.3 \\
Flowers & 95.0 $ \pm $ 0.1 & 94.1 $ \pm $ 0.3 & {N \slash A} & 76.0 $ \pm $ 1.3 & 94.9 $ \pm $ 0.3 & \textbf{96.0 $ \pm $ 0.0} & 93.0 $ \pm $ 0.3 & 95.0 $ \pm $ 0.3 \\
Food-101 & \textbf{87.3 $ \pm $ 0.1} & 85.5 $ \pm $ 0.0 & {N \slash A} & 85.4 $ \pm $ 0.1 & 85.1 $ \pm $ 0.2 & 86.6 $ \pm $ 0.0 & 83.0 $ \pm $ 0.1 & 86.3 $ \pm $ 0.1 \\
Pets & \textbf{93.4 $ \pm $ 0.1} & 91.0 $ \pm $ 0.1 & {N \slash A} & 84.5 $ \pm $ 0.5 & 90.1 $ \pm $ 0.2 & 91.6 $ \pm $ 0.3 & 89.9 $ \pm $ 0.3 & 92.3 $ \pm $ 0.3 \\
SUN397 & \textbf{64.8 $ \pm $ 0.0} & 61.4 $ \pm $ 0.2 & {N \slash A} & 51.4 $ \pm $ 0.3 & 60.0 $ \pm $ 0.3 & 61.1 $ \pm $ 0.2 & 59.0 $ \pm $ 0.1 & 60.9 $ \pm $ 0.1 \\


\midrule
{98\% Sparsity} & {} & {} & {} & {} & {} & {} & {} & {} \\
\midrule
Aircraft & \textbf{83.6 $ \pm $ 0.4} & 79.1 $ \pm $ 0.2 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 72.0 $ \pm $ 0.2 & 81.4 $ \pm $ 0.3 \\
Birds & \textbf{72.4 $ \pm $ 0.3} & 63.4 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 54.1 $ \pm $ 0.1 & 65.4 $ \pm $ 0.3 \\
CIFAR-10 & \textbf{97.4 $ \pm $ 0.0} & 95.0 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 93.8 $ \pm $ 0.1 & 96.0 $ \pm $ 0.0 \\
CIFAR-100 & \textbf{85.6 $ \pm $ 0.2} & 79.8 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 75.9 $ \pm $ 0.2 & 80.7 $ \pm $ 0.2 \\
Caltech-101 & \textbf{93.5 $ \pm $ 0.1} & 88.9 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 85.2 $ \pm $ 0.6 & 89.8 $ \pm $ 0.3 \\
Caltech-256 & \textbf{86.1 $ \pm $ 0.1} & 80.3 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 74.2 $ \pm $ 0.0 & 78.9 $ \pm $ 0.1 \\
Cars & \textbf{90.3 $ \pm $ 0.2} & 85.5 $ \pm $ 0.2 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 79.9 $ \pm $ 0.5 & 86.8 $ \pm $ 0.1 \\
DTD & \textbf{76.2 $ \pm $ 0.3} & 72.6 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 69.4 $ \pm $ 0.3 & 71.8 $ \pm $ 0.1 \\
Flowers & \textbf{95.0 $ \pm $ 0.1} & 92.9 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 91.8 $ \pm $ 0.3 & 94.0 $ \pm $ 0.2 \\
Food-101 & \textbf{87.3 $ \pm $ 0.1} & 83.2 $ \pm $ 0.0  & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 77.9 $ \pm $ 0.1 & 84.2 $ \pm $ 0.1 \\
Pets & \textbf{93.4 $ \pm $ 0.1} & 88.8 $ \pm $ 0.2 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 85.5 $ \pm $ 0.1 & 89.8 $ \pm $ 0.1 \\
SUN397 & \textbf{64.8 $ \pm $ 0.0} & 58.4 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 53.8 $ \pm $ 0.2 & 58.5 $ \pm $ 0.1 \\
\bottomrule
\end{tabular}

}
\caption{Transfer accuracy for sparse ResNet50 transfer with \emph{full finetuning}.}
\label{table:rn50_full_all}
\end{table}

==> tables/rn50_linear_all.tex <==
% RN 50 linear finetuning full results

\begin{table}[htb!]
\centering

\scalebox{0.9}{%
\begin{tabular}{ccccccccc}
\toprule
{Pruning Strategy} & {Dense} & {AC/DC} & {GMP} & {LTH-T} & {RigL ERK 1x} & {RigL ERK 5x} & {STR} & {WoodFisher} \\

\midrule
{80\% Sparsity} & {} & {} & {} & {} & {} & {} & {}\\
\midrule
Aircraft & 49.2 $ \pm $ 0.1 & \textbf{55.1 $ \pm $ 0.1} & 45.8 $ \pm $ 0.1 & 36.9 $ \pm $ 0.1 & 54.6 $ \pm $ 0.1 & \textbf{55.2 $ \pm $ 0.2} & 53.7 $ \pm $ 0.0 & 40.0 $ \pm $ 0.2 \\
Birds & 57.7 $ \pm $ 0.1 & \textbf{58.4 $ \pm $ 0.0} & 56.2 $ \pm $ 0.0 & 29.6 $ \pm $ 0.1 & 55.2 $ \pm $ 0.0 & 56.7 $ \pm $ 0.1 & 56.2 $ \pm $ 0.1 & 51.9 $ \pm $ 0.1 \\
CIFAR-10 & 91.2 $ \pm $ 0.0 & 90.9 $ \pm $ 0.0 & 89.7 $ \pm $ 0.0 & 83.4 $ \pm $ 0.1 & 89.7 $ \pm $ 0.1 & 90.0 $ \pm $ 0.1 & \textbf{91.4 $ \pm $ 0.0} & 89.6 $ \pm $ 0.0 \\
CIFAR-100 & \textbf{74.6 $ \pm $ 0.1} & \textbf{74.7 $ \pm $ 0.1} & 72.0 $ \pm $ 0.1 & 62.0 $ \pm $ 0.1 & 73.1 $ \pm $ 0.1 & 73.7 $ \pm $ 0.0 & \textbf{74.7 $ \pm $ 0.0} & 71.3 $ \pm $ 0.0 \\
Caltech-101 & 91.9 $ \pm $ 0.1 & \textbf{92.4 $ \pm $ 0.2} & 91.5 $ \pm $ 0.2 & 75.4 $ \pm $ 0.1 & 91.1 $ \pm $ 0.1 & 90.8 $ \pm $ 0.3 & 91.2 $ \pm $ 0.1 & 91.2 $ \pm $ 0.1 \\
Caltech-256 & \textbf{84.8 $ \pm $ 0.1} & \textbf{84.6 $ \pm $ 0.1} & 83.9 $ \pm $ 0.1 & 66.1 $ \pm $ 0.1 & 83.3 $ \pm $ 0.1 & \textbf{84.6 $ \pm $ 0.1} & 83.6 $ \pm $ 0.0 & 83.7 $ \pm $ 0.1 \\
Cars & 53.4 $ \pm $ 0.1 & 56.6 $ \pm $ 0.0 & 49.1 $ \pm $ 0.1 & 32.7 $ \pm $ 0.1 & 57.4 $ \pm $ 0.1 & \textbf{58.6 $ \pm $ 0.1} & 57.0 $ \pm $ 0.1 & 44.9 $ \pm $ 0.1 \\
DTD & 73.5 $ \pm $ 0.2 & \textbf{74.4 $ \pm $ 0.1} & 71.2 $ \pm $ 0.1 & 64.9 $ \pm $ 0.2 & 73.5 $ \pm $ 0.2 & 72.9 $ \pm $ 0.3 & \textbf{74.3 $ \pm $ 0.2} & 70.8 $ \pm $ 0.2 \\
Flowers & 91.6 $ \pm $ 0.1 & 92.7 $ \pm $ 0.1 & 90.9 $ \pm $ 0.1 & 85.6 $ \pm $ 0.1 & 92.2 $ \pm $ 0.1 & 92.3 $ \pm $ 0.1 & \textbf{93.0 $ \pm $ 0.0} & 87.6 $ \pm $ 0.1 \\
Food-101 & 73.2 $ \pm $ 0.0 & 73.8 $ \pm $ 0.0 & 70.5 $ \pm $ 0.0 & 61.9 $ \pm $ 0.0 & 73.3 $ \pm $ 0.0 & 72.5 $ \pm $ 0.1 & \textbf{73.9 $ \pm $ 0.0} & 68.5 $ \pm $ 0.0 \\
Pets & \textbf{92.6 $ \pm $ 0.1} & 92.3 $ \pm $ 0.1 & \textbf{92.5 $ \pm $ 0.1} & 79.4 $ \pm $ 0.1 & 91.9 $ \pm $ 0.1 & \textbf{92.5 $ \pm $ 0.2} & 91.7 $ \pm $ 0.0 & 92.2 $ \pm $ 0.1 \\
SUN397 & 60.1 $ \pm $ 0.0 & \textbf{60.4 $ \pm $ 0.0} & 58.1 $ \pm $ 0.0 & 47.4 $ \pm $ 0.0 & 59.1 $ \pm $ 0.1 & 59.9 $ \pm $ 0.0 & 60.3 $ \pm $ 0.0 & 57.8 $ \pm $ 0.1 \\

\midrule
{90\% Sparsity} & {} & {} & {} & {} & {} & {} & {}\\
\midrule
Aircraft & 49.2 $ \pm $ 0.1 & 55.5 $ \pm $ 0.1 & 48.7 $ \pm $ 0.1 & 16.5 $ \pm $ 0.2 & 54.1 $ \pm $ 0.1 & \textbf{56.6 $ \pm $ 0.1} & 52.9 $ \pm $ 0.1 & 44.0 $ \pm $ 0.2 \\
Birds & 57.7 $ \pm $ 0.1 & \textbf{58.7 $ \pm $ 0.0} & 55.4 $ \pm $ 0.1 & 11.4 $ \pm $ 0.1 & 53.3 $ \pm $ 0.0 & 57.2 $ \pm $ 0.1 & 55.2 $ \pm $ 0.1 & 52.7 $ \pm $ 0.1 \\
CIFAR-10 & \textbf{91.2 $ \pm $ 0.0} & 91.0 $ \pm $ 0.0 & 89.4 $ \pm $ 0.0 & 67.0 $ \pm $ 0.1 & 90.0 $ \pm $ 0.1 & 90.2 $ \pm $ 0.1 & 90.6 $ \pm $ 0.0 & 88.9 $ \pm $ 0.0 \\
CIFAR-100 & \textbf{74.6 $ \pm $ 0.1} & 74.3 $ \pm $ 0.0 & 71.5 $ \pm $ 0.0 & 42.2 $ \pm $ 0.1 & 72.8 $ \pm $ 0.1 & 73.4 $ \pm $ 0.1 & 73.7 $ \pm $ 0.1 & 70.5 $ \pm $ 0.0 \\
Caltech-101 & 91.9 $ \pm $ 0.1 & \textbf{92.5 $ \pm $ 0.1} & 91.6 $ \pm $ 0.1 & 49.0 $ \pm $ 0.6 & 90.6 $ \pm $ 0.3 & 91.4 $ \pm $ 0.4 & 90.9 $ \pm $ 0.1 & 91.3 $ \pm $ 0.1 \\
Caltech-256 & \textbf{84.8 $ \pm $ 0.1} & 84.5 $ \pm $ 0.0 & 82.9 $ \pm $ 0.0 & 42.0 $ \pm $ 0.1 & 81.9 $ \pm $ 0.0 & 84.5 $ \pm $ 0.1 & 82.6 $ \pm $ 0.0 & 83.0 $ \pm $ 0.1 \\
Cars & 53.4 $ \pm $ 0.1 & 56.0 $ \pm $ 0.1 & 50.2 $ \pm $ 0.0 & 15.4 $ \pm $ 0.1 & 55.5 $ \pm $ 0.1 & \textbf{60.5 $ \pm $ 0.1} & 54.8 $ \pm $ 0.1 & 46.7 $ \pm $ 0.0 \\
DTD & \textbf{73.5 $ \pm $ 0.2} & \textbf{73.7 $ \pm $ 0.2} & 72.4 $ \pm $ 0.2 & 54.7 $ \pm $ 0.1 & 72.6 $ \pm $ 0.3 & 72.7 $ \pm $ 0.2 & \textbf{73.8 $ \pm $ 0.1} & 71.0 $ \pm $ 0.2 \\
Flowers & 91.6 $ \pm $ 0.1 & 92.4 $ \pm $ 0.0 & 91.4 $ \pm $ 0.1 & 67.7 $ \pm $ 0.1 & 91.6 $ \pm $ 0.1 & 92.4 $ \pm $ 0.1 & \textbf{93.0 $ \pm $ 0.1} & 89.0 $ \pm $ 0.1 \\
Food-101 & 73.2 $ \pm $ 0.0 & \textbf{73.8 $ \pm $ 0.0} & 71.1 $ \pm $ 0.0 & 46.9 $ \pm $ 0.0 & 71.7 $ \pm $ 0.0 & 72.6 $ \pm $ 0.0 & 72.6 $ \pm $ 0.0 & 69.2 $ \pm $ 0.0 \\
Pets & \textbf{92.6 $ \pm $ 0.1} & 91.9 $ \pm $ 0.1 & 92.0 $ \pm $ 0.1 & 43.8 $ \pm $ 0.2 & 91.1 $ \pm $ 0.1 & 91.9 $ \pm $ 0.2 & 91.1 $ \pm $ 0.1 & 92.0 $ \pm $ 0.1 \\
SUN397 & \textbf{60.1 $ \pm $ 0.0} & 59.8 $ \pm $ 0.1 & 58.1 $ \pm $ 0.0 & 31.7 $ \pm $ 0.1 & 57.7 $ \pm $ 0.0 & 59.8 $ \pm $ 0.1 & 58.2 $ \pm $ 0.0 & 56.8 $ \pm $ 0.0 \\


\midrule
{95\% Sparsity} & {} & {} & {} & {} & {} & {} & {}\\
\midrule
Aircraft & 49.2 $ \pm $ 0.1 & 56.6 $ \pm $ 0.1 & {N \slash A} & 4.5 $ \pm $ 0.3 & 53.5 $ \pm $ 0.1 & \textbf{56.9 $ \pm $ 0.1} & 50.3 $ \pm $ 0.1 & 45.6 $ \pm $ 0.3 \\
Birds & \textbf{57.7 $ \pm $ 0.1} & \textbf{57.7 $ \pm $ 0.0} & {N \slash A} & 2.3 $ \pm $ 0.1 & 51.9 $ \pm $ 0.1 & 55.9 $ \pm $ 0.0 & 52.1 $ \pm $ 0.1 & 51.8 $ \pm $ 0.1 \\
CIFAR-10 & \textbf{91.2 $ \pm $ 0.0} & 90.5 $ \pm $ 0.0 & {N \slash A} & 39.9 $ \pm $ 0.2 & 89.4 $ \pm $ 0.0 & 89.8 $ \pm $ 0.1 & 89.1 $ \pm $ 0.0 & 88.6 $ \pm $ 0.0 \\
CIFAR-100 & \textbf{74.6 $ \pm $ 0.1} & 73.4 $ \pm $ 0.0 & {N \slash A} & 13.5 $ \pm $ 0.2 & 71.5 $ \pm $ 0.1 & 72.4 $ \pm $ 0.1 & 71.7 $ \pm $ 0.0 & 69.7 $ \pm $ 0.0 \\
Caltech-101 & \textbf{91.9 $ \pm $ 0.1} & 91.6 $ \pm $ 0.1 & {N \slash A} & 20.1 $ \pm $ 0.5 & 89.0 $ \pm $ 0.1 & 91.4 $ \pm $ 0.1 & 90.0 $ \pm $ 0.2 & 91.0 $ \pm $ 0.2 \\
Caltech-256 & \textbf{84.8 $ \pm $ 0.1} & 82.8 $ \pm $ 0.1 & {N \slash A} & 12.4 $ \pm $ 0.3 & 80.1 $ \pm $ 0.1 & 83.5 $ \pm $ 0.1 & 80.2 $ \pm $ 0.1 & 81.2 $ \pm $ 0.1 \\
Cars & 53.4 $ \pm $ 0.1 & \textbf{56.9 $ \pm $ 0.1} & {N \slash A} & 3.9 $ \pm $ 0.1 & 52.9 $ \pm $ 0.0 & \textbf{57.0 $ \pm $ 0.1} & 50.5 $ \pm $ 0.1 & 45.5 $ \pm $ 0.0 \\
DTD & \textbf{73.5 $ \pm $ 0.2} & 72.7 $ \pm $ 0.1 & {N \slash A} & 27.4 $ \pm $ 0.2 & 71.9 $ \pm $ 0.1 & 72.9 $ \pm $ 0.2 & 72.1 $ \pm $ 0.2 & 70.4 $ \pm $ 0.1 \\
Flowers & 91.6 $ \pm $ 0.1 & \textbf{93.0 $ \pm $ 0.1} & {N \slash A} & 27.8 $ \pm $ 0.6 & 91.0 $ \pm $ 0.1 & 92.4 $ \pm $ 0.1 & 91.9 $ \pm $ 0.1 & 89.6 $ \pm $ 0.0 \\
Food-101 & \textbf{73.2 $ \pm $ 0.0} & \textbf{73.2 $ \pm $ 0.0} & {N \slash A} & 15.0 $ \pm $ 0.1 & 70.6 $ \pm $ 0.1 & 71.9 $ \pm $ 0.0 & 70.7 $ \pm $ 0.0 & 68.2 $ \pm $ 0.0 \\
Pets & \textbf{92.6 $ \pm $ 0.1} & 91.0 $ \pm $ 0.2 & {N \slash A} & 15.9 $ \pm $ 0.2 & 90.1 $ \pm $ 0.1 & 91.1 $ \pm $ 0.1 & 89.8 $ \pm $ 0.1 & 91.4 $ \pm $ 0.0 \\
SUN397 & \textbf{60.1 $ \pm $ 0.0} & 58.2 $ \pm $ 0.0 & {N \slash A} & 8.4 $ \pm $ 0.2 & 55.9 $ \pm $ 0.1 & 58.3 $ \pm $ 0.1 & 56.3 $ \pm $ 0.0 & 55.1 $ \pm $ 0.1 \\

\midrule
{98\% Sparsity} & {} & {} & {} & {} & {} & {} \\
\midrule
Aircraft & 49.2 $ \pm $ 0.1 & \textbf{54.8 $ \pm $ 0.1} & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 48.0 $ \pm $ 0.1 & 45.0 $ \pm $ 0.1 \\
Birds & \textbf{57.7 $ \pm $ 0.1} & 54.5 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 43.7 $ \pm $ 0.0 & 48.1 $ \pm $ 0.1 \\
CIFAR-10 & \textbf{91.2 $ \pm $ 0.0} & 89.2 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 86.5 $ \pm $ 0.0 & 86.6 $ \pm $ 0.0 \\
CIFAR-100 & \textbf{74.6 $ \pm $ 0.1} & 71.6 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 67.4 $ \pm $ 0.0 & 67.8 $ \pm $ 0.0 \\
Caltech-101 & \textbf{91.9 $ \pm $ 0.1} & 89.0 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 86.3 $ \pm $ 0.1 & 88.5 $ \pm $ 0.1 \\
Caltech-256 & \textbf{84.8 $ \pm $ 0.1} & 79.8 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 73.4 $ \pm $ 0.1 & 77.1 $ \pm $ 0.0 \\
Cars & \textbf{53.4 $ \pm $ 0.1} & 52.1 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 44.4 $ \pm $ 0.1 & 42.2 $ \pm $ 0.0 \\
DTD & \textbf{73.5 $ \pm $ 0.2} & 71.6 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 68.4 $ \pm $ 0.2 & 68.3 $ \pm $ 0.1 \\
Flowers & 91.6 $ \pm $ 0.1 & \textbf{92.3 $ \pm $ 0.1} & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 90.8 $ \pm $ 0.1 & 89.5 $ \pm $ 0.1 \\
Food-101 & \textbf{73.2 $ \pm $ 0.0} & 70.8 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 65.3 $ \pm $ 0.0 & 66.5 $ \pm $ 0.0 \\
Pets & \textbf{92.6 $ \pm $ 0.1} & 89.2 $ \pm $ 0.1 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 85.5 $ \pm $ 0.1 & 88.7 $ \pm $ 0.1 \\
SUN397 & \textbf{60.1 $ \pm $ 0.0} & 55.1 $ \pm $ 0.0 & {N \slash A} & {N \slash A} & {N \slash A} & {N \slash A} & 50.9 $ \pm $ 0.0 & 52.4 $ \pm $ 0.0 \\
\bottomrule
\end{tabular}
}
\caption{Transfer accuracy for sparse ResNet50 transfer with \emph{linear finetuning}.}
\label{table:rn50_linear_all}
\end{table}


==> tables/segmentation_dense.tex <==
\begin{table}[t!]
\centering
\scalebox{0.9}{%
\begin{tabular}{c|ccccccccccc}
\toprule
{Type} & all & 0.5 & 0.55 & 0.6 & 0.65 & 0.7 & 0.75 & 0.8 & 0.85 & 0.9 & 0.95 \\
\midrule
box & 32.62 & 54.05 & 51.96 & 48.72 & 44.81 & 40.84 & 34.72 & 26.89 & 17.33 & 6.33 & 0.55 \\
mask & 30.74 & 50.28 & 47.66 & 44.57 & 41.02 & 36.39 & 31.47 & 25.53 & 18.55 & 10.03 & 1.91 \\
\bottomrule
\end{tabular}
}
\caption{Mean average precision for dense transfer on Pascal, at various thresholds.}
\label{table:segmentation_dense}
\end{table}

==> tables/segmentation_sparse.tex <==
\begin{table}[t!]
\centering
\scalebox{0.9}{%
\begin{tabular}{c|ccccccccccc}
\toprule
{Type} & all & 0.5 & 0.55 & 0.6 & 0.65 & 0.7 & 0.75 & 0.8 & 0.85 & 0.9 & 0.95 \\
\midrule
box & 33.55 & 54.15 & 51.79 & 49.2 & 45.57 & 41.51 & 35.95 & 29.2 & 19.66 & 7.78 & 0.74 \\
mask & 31.5 & 50.66 & 47.89 & 45.04 & 41.67 & 37.32 & 32.39 & 26.35 & 19.98 & 11.22 & 2.5 \\
\bottomrule
\end{tabular}
}
\caption{Mean average precision for \emph{sparse} transfer on Pascal, at various thresholds. Notice the similar or slightly improved accuracy.}
\label{table:segmentation_sparse}
\end{table}
